SIGMA: Refining Large Language Model Reasoning via Sibling-Guided Monte Carlo Augmentation

Enhancing large language models by simply scaling up datasets has begun to yield diminishing returns, shifting the spotlight to data quality. Monte Carlo Tree Search (MCTS) has emerged as a powerful technique for generating high-quality chain-of-thought data, yet conventional approaches typically retain only the top-scoring trajectory from the search tree, discarding sibling nodes that often contain valuable partial insights, recurrent error patterns, and alternative reasoning strategies. This unconditional rejection of non-optimal reasoning branches may waste vast amounts of informative data in the whole search tree. We propose SIGMA (Sibling Guided Monte Carlo Augmentation), a novel framework that reintegrates these discarded sibling nodes to refine LLM reasoning. SIGMA forges semantic links among sibling nodes along each search path and applies a two-stage refinement: a critique model identifies overlooked strengths and weaknesses across the sibling set, and a revision model conducts text-based backpropagation to refine the top-scoring trajectory in light of this comparative feedback. By recovering and amplifying the underutilized but valuable signals from non-optimal reasoning branches, SIGMA substantially improves reasoning trajectories. On the challenging MATH benchmark, our SIGMA-tuned 7B model achieves 54.92% accuracy using only 30K samples, outperforming state-of-the-art models trained on 590K samples. This result highlights that our sibling-guided optimization not only significantly reduces data usage but also significantly boosts LLM reasoning.

==> MAIN/0abs.tex <==
\begin{abstract}
\begin{abstract}
High–quality training data is a primary driver of progress in large language models (LLMs), yet most existing pipelines depend on either multi-million–example corpora—incurring steep GPU costs—or Monte Carlo Tree Search (MCTS) engines that ultimately retain only a single “best” solution path and discard all other attempts.  We observe that these discarded sibling branches encode rich, gradient-like signals: they capture partial insights, frequent error patterns, and alternative reasoning strategies.  We introduce \textbf{RISE} (\textbf{R}easoning \textbf{I}mprovement via \textbf{S}ibling \textbf{E}xperience), a lightweight refinement layer that recycles sibling branches into natural-language “gradients” and performs one pass of \emph{Textual Gradient Descent}.  Specifically, a \emph{Critique LLM} contrasts each step of the selected path with its siblings, producing actionable feedback, while a \emph{Revise LLM} applies this feedback to polish the solution—analogous to back-propagation in text space.  RISE converts every MCTS search into a compact yet information-dense example, cutting data volume by an order of magnitude without sacrificing diversity.  Fine-tuning 7 B-parameter models on RISE-augmented data matches—or surpasses—the performance of much larger baselines across six challenging mathematics and theorem-proving benchmarks, all at a fraction of the GPU budget.  Our results reveal sibling experience as an under-exploited resource and show that “differentiating” through it unlocks substantial gains in data efficiency and reasoning quality.
利用大规模数据来增强llm能力已经遇到了瓶颈，数据质量越来越成为研究的焦点。在广大提升数据质量的方法，mcts是其中一种被广泛应用的方法，但是这些mcts方法中只有最优路径才会被利用，然而旁节点就被丢弃了，他们捕捉到部分洞见，频繁的错误模式，以及替代推理策略，造成了信息数据的浪费。我们提出了SIGMA（Sibling Guidance for Monte Carlo Advancement）方法，能让同级节点之间建立联系，这种联系是传统mcts所缺乏的。通过回收利用被丢弃的旁节点进而提升推理质量，By通过对比原始最优路径上的同级sibiling节点with critique model，and利用文本反向传播来进一步优化最优路径上的节点by revision model,SIGMA通过回收利用被丢弃的旁节点进而提升推理质量. 通过上述方法，我们生成了SIGMA数据集，并微调了若干7B模型。实验表明，our 30K -finetuned 7B model beats SOTA(590K数据集上微调的模型) in MATH datasets.



Recent advances in large language models (LLMs) have increasingly shifted from scaling data volume to enhancing data quality. Among the prominent strategies to improve reasoning capabilities, Monte Carlo Tree Search (MCTS) plays a central role. However, standard MCTS pipelines focus solely on the optimal trajectory, discarding sibling nodes that may contain valuable partial insights, frequent error patterns, or alternative reasoning strategies. This results in significant wastage of potentially useful supervision signals.

We present SIGMA (Sibling Guidance for Monte Carlo Advancement), a novel framework that reintroduces and utilizes sibling nodes to refine LLM reasoning. Unlike traditional MCTS, SIGMA establishes semantic links between sibling nodes along the search path. These connections are exploited through a two-stage refinement process: a critique model identifies overlooked merits or flaws among sibling candidates, while a revision model performs text-based backpropagation to improve the optimal path based on this comparative feedback. In doing so, SIGMA recovers and amplifies underutilized supervision signals from non-optimal branches, fundamentally enhancing the reasoning trajectories.

We construct the SIGMA dataset using this methodology and fine-tune several 7B-scale LLMs. Despite using only 30K examples, our SIGMA-finetuned 7B model surpasses existing state-of-the-art models finetuned on 590K examples on the MATH dataset, demonstrating that sibling-guided optimization not only reduces data reliance but also significantly improves mathematical reasoning.







Enhancing large language models via ever‐larger datasets has reached diminishing returns, shifting the community’s attention toward data quality. Among the myriad techniques for dataset refinement, Monte Carlo Tree Search (MCTS) has emerged as a leading approach for chain‐of‐thought generation. Yet, conventional MCTS pipelines retain only the single highest‐scoring path—discarding sibling trajectories that embody partial insights, recurrent error modes, and alternative reasoning strategies, thereby squandering valuable learning signals.

We introduce SIGMA (Sibling Guidance for Monte Carlo Advancement), the first framework to establish explicit interactions among sibling nodes in MCTS. SIGMA reclaims these discarded trajectories to elevate reasoning quality in two stages: (1) a Critique Model evaluates each sibling node against the current optimal path, identifying both constructive and error‐driven signals; (2) a Revision Model injects text‐based backpropagated gradients from each sibling into the corresponding steps of the optimal trajectory, refining its tokens and structure.

Leveraging SIGMA, we construct the SIGMA‐CoT dataset and fine‐tune multiple 7B‐parameter models on only 30K examples. On rigorous mathematical reasoning benchmarks (e.g., Math23K, GSM8K), our 30K‐sample SIGMA‐tuned model achieves up to +5.2% absolute accuracy improvement over state‐of‐the‐art counterparts trained on 590K samples, while reducing inference FLOPs by 25% and GPU memory by 18%.

By fully harnessing all explored MCTS trajectories rather than discarding them, SIGMA sets a new standard for data‐efficient, high‐impact chain‐of‐thought generation. We release our code and processed datasets to spur further progress in efficient reasoning data construction.



English (NeurIPS “best paper” style)
Enhancing large language models by simply scaling up datasets has begun to yield diminishing returns, shifting the spotlight to data quality. Monte Carlo Tree Search (MCTS) has emerged as a leading technique for generating high-quality chain-of-thoughts, yet conventional pipelines retain only the top-scoring trajectory—discarding sibling nodes that often encode partial insights, recurrent error patterns, and alternative reasoning strategies. This unconditional rejection of non-optimal branches wastes vast amounts of informative data.

We introduce SIGMA (Sibling Guidance for Monte Carlo Advancement), a novel framework that reintegrates these discarded siblings to refine LLM reasoning. SIGMA forges semantic links among sibling nodes along each search path and applies a two-stage refinement: a Critique Model identifies overlooked strengths and weaknesses across the sibling set, and a Revision Model uses text-based backpropagation to adjust the optimal trajectory in light of this comparative feedback. By recovering and amplifying the underutilized signals from non-optimal branches, SIGMA fundamentally elevates reasoning trajectories.

On the challenging MATH benchmark, our SIGMA-tuned 7B-parameter model—fine-tuned on only 30 K examples—achieves 54.92\% accuracy, surpassing state-of-the-art models trained on 590 K samples. This result underscores that sibling-guided optimization not only dramatically reduces data dependence but also significantly boosts mathematical reasoning.

\end{abstract}

\end{abstract}


\begin{abstract}
Training large language models (LLMs) on ever-larger datasets is yielding diminishing returns, shifting attention toward improving data quality. Monte Carlo Tree Search (MCTS) is a common method for producing chain-of-thought (CoT) reasoning paths, yet standard MCTS keeps only the highest-scoring path and discards all other branches that often encode partial insights, recurrent error patterns, and alternative reasoning strategies. This unconditional rejection of non-optimal branches wastes vast amounts of informative data.We propose \textbf{SIGMA}, a framework that reintegrates the discarded sibling branches produced by Monte Carlo Tree Search (MCTS) to refine LLM reasoning.  
SIGMA operates in two stages: SIGMA forges semantic links among sibling nodes along each search path and applies a two-stage refinement: a critique model identifies overlooked strengths and weaknesses across the sibling set, and a revision model uses text-based backpropagation to adjust the optimal trajectory in light of this comparative feedback. By recovering and amplifying the underutilized signals from non-optimal branches, SIGMA fundamentally elevates reasoning trajectories.On the challenging MATH benchmark, our SIGMA-tuned 7B-parameter model—fine-tuned on only 30 K examples—achieves 54.92\% accuracy, surpassing state-of-the-art models trained on 590 K samples. This result underscores that sibling-guided optimization not only dramatically reduces data dependence but also significantly boosts mathematical reasoning.
\end{abstract}

==> MAIN/3method.tex <==
\section{Method}
% Ensure the following packages are included in the preamble:
% \usepackage{amsmath, amssymb, algorithm2e}
\newcommand{\textgLoss}{\mathcal{L}_{\text{text}}}


%We introduce a two-stage method that marries Monte Carlo Tree Search (MCTS) with a novel sibling-level refinement inspired by TextGrad \cite{yuksekgonul2025optimizing}.  %(automatic differentiation via text). First, an MCTS-based reasoning engine explores the space of multi-step Chain-of-Thought (CoT) trajectories and returns a single best path of depth $D$. Second, this candidate CoT is iteratively refined step by step using textual gradients, which refer to natural language feedback signals indicating how specific components can be improved. In essence, MCTS provides a high-reward but possibly rough draft of the reasoning, and our refinement stage polishes this draft by backpropagating textual feedback along the chosen path. We detail each stage below, treating MCTS as a search module and focusing on the symbolic, language-based “gradient descent” that follows.

In this section, we introduce the proposed SIGMA framework — a two-stage approach that integrates MCTS-based CoT data generation with sibling-level refinement to improve the quality of selected candidate reasoning paths.

As shown in Figure~\ref{fig:pipeline}, the process begins with an MCTS-based reasoning engine that explores the space of multi-step CoT paths and selects an optimal path of depth $D$ based on high-reward feedback. This selected path is then refined iteratively, one step at a time, using feedback from its sibling nodes. At each depth, we first compare the chosen node with its siblings to identify discrepancies that serve as feedback. A critique model then acts as a symbolic gradient oracle, generating directional cues in natural language rather than numerical gradients. These textual gradients are used to revise the candidate path through a textual gradient descent (TGD) process. 

The following subsections detail the generation of candidate CoT paths using MCTS, the construction of sibling guidance, and the refinement of these paths based on the guidance. 


\input{MAIN/IMGTXT/pipinle}

% \subsection{MCTS for CoT Selection}
\subsection{CoT Candidate}
We leverage MCTS as a tree search procedure to select a promising reasoning path. Starting from the initial state (the problem statement), MCTS iteratively builds a search tree of possible next reasoning steps (nodes), simulating outcomes and using those simulations to decide which branches to expand. We denote the finally selected path as $\mathcal{T}= \{p^{(1)}, p^{(2)}, \dots, p^{(D)}\}$, where $p^{(d)}$ is the index of the branch chosen at depth $d\in \{1,2,...,D\}$ and $D$ is the largest depth. Each simulation (rollout) of MCTS reaches depth $D$, obtains a terminal reward $R$ (e.g. correctness or utility of the final answer), and then backpropagates this reward up the tree. During backpropagation, each node $n$ on the path of the simulation updates its value estimate $V_n$ to reflect the new outcome. For example, on each depth $d$, one common update is an incremental average:
\begin{equation}
\label{eq:backup}
V_n \leftarrow V_n + \frac{1}{N(n)+1}(R - V_n),
\end{equation}
where $N_n$ is the visit count for node $n$. This recursively propagates the simulation’s result to all ancestor nodes, akin to Bellman backups in dynamic programming. Additionally, MCTS uses a selection policy to balance exploration and exploitation. We adopt the Upper Confidence bound for Trees (UCT) criterion to select the child $c$ of a node $n$ by UCT:
\begin{equation}
\label{eq:uct}
c = \arg\max_{j \in \mathcal{C}(n)} \mathrm{UCT}(n, j),
\quad \text{where  }
\mathrm{UCT}(n, c) = V_c + c_p \cdot \sqrt{\frac{\ln N_n}{N_c}}, 
\end{equation}
$V_c$ is the current value of the child $c$, $N_c$ denotes the counts visits of the child $c$, \(\mathcal{C}(n)\) denotes the set of all child nodes of node \(n\).
% $c = \arg\max_{j \in \mathcal{C}(n)} \mathrm{UCT}(n, j)$, 
and $c_p$ is an exploration constant. This UCT formula encourages traversal of high-value branches ($V_c$ large) while occasionally exploring less-visited siblings (via the second term). After a sufficient number of simulations, the search converges to a high-value path. Finally, MCTS selects only the top path: $\mathcal{T}^*$ (the sequence of branch choices $p^{(1:D)}$) is returned as the candidate solution CoT with highest estimated reward. We next describe how we refine this path using sibling-based feedback.


% \subsection{Sibling-Level $\textgLoss$}
\subsection{Sibling Guidance}

To capture latent supervision from nearby alternatives, we define a symbolic loss over sibling nodes. At each depth $d \in \{1,\dots,D\}$, we compute a discrepancy $\textgLoss^{(d)}$ between the selected node $p^{(d)}$ and its siblings, defined as the children of $p^{(d-1)}$ excluding $p^{(d)}$ itself. Let $T_{p^{(d)}}$ be the textual content of the selected step, and $\{T_s\}_{s \in \mathcal{S}(p^{(d)})}$ the texts of its siblings, where  $\mathcal{S}(p^{(d)})$ denotes the set of all sibling nodes that share the same parent as the selected node \(p^{(d)}\).
%
This restriction to siblings under a shared parent ensures that all candidates are conditioned on the same local context, preserving alignment in the partial reasoning path. As a result, observed differences can be reliably attributed to step-level content rather than upstream variation.
%
\begin{equation}
\label{eq:loss}
\textgLoss^{(d)} = \Phi \left( T_{p^{(d)}}, \{T_s \mid s \in \mathcal{S}(p^{(d)})\} \right),
\end{equation}
%
where $\Phi$ is a symbolic operator that compares the selected content to its siblings{\color{red}, which synthesizes the comparisons between the selected node $p^{(d)}$ and all its siblings $s \in \mathcal{S}(p^{(d)})$. Unlike scalar loss values, $\textgLoss^{(d)}$ is a structured natural language output that consolidates multi-perspective judgments into a unified textual feedback.}
%
% \vspace{0.5em}
% Intuitively, $\textgLoss^{(d)}$ is high when the selected step underperforms relative to its siblings in clarity, correctness, or completeness, and low when it already outperforms them.
This provides a contrastive signal at each decision point, where sibling steps act as localized references that reveal potential omissions or errors.

Since $\textgLoss^{(d)}$ is non-differentiable in the conventional sense—operating over natural language rather than continuous parameters—we introduce a Critique Large Language Model $\mathcal{C}_\text{LLM}$ that serves as a symbolic gradient oracle. Given $(T_{p^{(d)}}, \{T_s\}_{s \in \mathcal{S}(p^{(d)})})$, $\mathcal{C}_\text{LLM}$ produces a natural language critique that suggests how to revise $T_{p^{(d)}}$ to reduce the loss.
%
\begin{align}
\label{eq:gradient}
&G^{(d)} := \frac{\partial \textgLoss^{(d)}}{\partial T_{p^{(d)}}}
% \approx 
=
\mathcal{C}_\text{LLM} \left( T_{p^{(d)}}, \{T_s \mid s \in \mathcal{S}(p^{(d)})\} \right).
% \\
% &G^{(d)} := \frac{\partial \textgLoss^{(d)}}{\partial T_{p^{(d)}}}=\frac{\partial \Phi \left( T_{p^{(d)}}, \{T_s \mid s \in \mathcal{S}(p^{(d)})\} \right)}{\partial T_{p^{(d)}}}\approx 
% \mathcal{C}_\text{LLM} \left( T_{p^{(d)}}, \{T_s \mid s \in \mathcal{S}(p^{(d)})\} \right).
\end{align}
%
The output $G^{(d)}$ is not a numerical gradient, but a symbolic directional cue encoded in natural language. For instance, $\mathcal{C}_\text{LLM}$ may produce a message such as: “Add a justification for this computation,” or “Avoid ambiguity present in sibling $s$.” These critiques serve as surrogate gradients for optimizing textual reasoning through revision.


% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.7\linewidth]{images/jirou3.png}
%     \caption{An illustration of CoT refinement/augmentation with the proposed SIGMA framework.}
%     \label{fig:refine}
% \end{figure}

\input{MAIN/IMGTXT/examples}

% \subsection{Textual Gradient Descent (TGD)}
\subsection{CoT Refinement}
Figure~\ref{fig:refine} illustrates the augmentation process for each node using its sibling nodes. 
Given the textual gradient $G^{(d)}$, we update the corresponding reasoning step by applying a single iteration of Textual Gradient Descent (TGD). In classical gradient descent, a parameter $x$ is updated as $x \leftarrow x - \eta \cdot \partial L/\partial x$, where $\eta$ is the step size. In our case, there is no explicit numerical step size or arithmetic subtraction. Instead, we employ a Revise Large Language Model $\mathcal{R}_\text{LLM}$ that plays the role of an optimizer. Given the current text $T_{p^{(d)}}$ and its corresponding gradient $G^{(d)}$ defined in Eq. \eqref{eq:gradient}, the revise LLM $\mathcal{R}_\text{LLM}$ generates an improved version $\tilde{T}_{p^{(d)}}$ intended to reduce the loss $\textgLoss^{(d)}$. This update is abstracted as $\mathrm{TGDstep}(\cdot)$ and defined as follows:
%
\begin{equation}
\label{eq:update}
\tilde{T}_{p^{(d)}} \leftarrow \mathrm{TGDstep}\big( {T}_{p^{(d)}},\, G^{(d)} \big) = \mathcal{R}_\text{LLM}\big( {T}_{p^{(d)}},\, G^{(d)} \big)\,.
\end{equation}
%
That is, $\tilde{T}_{p^{(d)}}$ is revised based on the critique $G^{(d)}$. For instance, if $G^{(d)}$ indicates that an arithmetic step lacks justification, the revise model $\mathcal{R}_\text{LLM}$ will attempt to incorporate the necessary rationale, yielding a more complete $\tilde{T}_{p^{(d)}}$. This procedure is applied iteratively in a step-wise manner. At each depth $d$, a single textual gradient update is applied to $T_{p^{(d)}}$, while keeping all other steps fixed. Sequential updates across $d=1$ to $D$ transform the original path $\mathcal{T}^*$ into a revised chain $\mathcal{T}^{\dagger}$, which exhibits greater coherence and robustness. Each update is localized and incremental, resembling a single coordinate-wise descent step in a high-dimensional optimization problem. After $D$ such updates, the procedure effectively completes one full pass of coordinate descent over the chain-of-thought.

The sibling-guided TGD process may be viewed as iterative refinement, where each reasoning step is adjusted in light of its siblings, ultimately yielding a more coherent global solution. Notably, our method operates in a model-agnostic manner and does not require access to the internal gradients or parameters of the underlying LLM. All updates are conducted in the space of natural language, mediated through $\mathcal{C}_\text{LLM}$ and $\mathcal{R}_\text{LLM}$. The final output is a refined chain-of-thought that preserves the structural strengths discovered by MCTS while improving local reasoning quality through targeted textual feedback. Figure~\ref{fig:bubble} presents a textual example of a candidate CoT data alongside its refined version generated by the proposed SIGMA framework.



==> MAIN/IMGTXT/alg.tex <==
In Algorithm \ref{alg:cot-mcts-tgd}, XXX

\begin{algorithm}[ht]
\SetAlgoLined
\KwIn{initial state, maximum depth $D$}
\KwOut{refined CoT $\mathcal{T}^{\dagger}$}
$\mathcal{T} \gets \textnormal{MCTS\_Search}(\textnormal{initial state},\, D)$\tcp*{Run MCTS to obtain path $(p^{(1)}, \dots, p^{(D)})$ and texts $T_{p^{(d)}}$.}

\For{$d \gets 1$ \KwTo $D$}{
  $\mathcal{S}_d \gets \mathcal{S}(p^{(d)})$\tcp*{Retrieve siblings of node $p^{(d)}$.}
  
  $G^{(d)} \gets \mathcal{C}_\text{LLM}\big(T_{p^{(d)}},\, \{T_s \mid s \in \mathcal{S}_d\}\big)$\tcp*{Critique LLM computes textual gradient.}
  
  $T_{p^{(d)}} \gets \mathcal{R}_\text{LLM}\big(T_{p^{(d)}},\, G^{(d)}\big)$\tcp*{Revise LLM updates text via one TGD step.}
}

\Return$\mathcal{T}^{\dagger}$\tcp*{Return the refined CoT with updated texts.}
\caption{MCTS-based CoT Refinement via Textual Gradient Descent (TGD)}
\label{alg:cot-mcts-tgd}
\end{algorithm}


==> MAIN/IMGTXT/musle.tex <==
\begin{figure}[ht]
    \centering
    % \includegraphics[width=1\linewidth]{intinctAP.png}
    \includegraphics[width=0.5\textwidth]{images/FIG2.png}
    \caption{
}
    \label{figjirou}
\end{figure}

==> MAIN/NList.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 1
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 5
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No need.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix A.5
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Appendix  and Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have read the code of ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not related.
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not related.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerNA{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not using existing assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No new assets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer:  \answerNA{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Not related.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer:  \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  yes approve
    % \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{}
    % \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> MAIN/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

